A comparison of limited-memory Krylov methods for Stieltjes functions of Hermitian matrices

Given a limited amount of memory and a target accuracy, we propose and compare several polynomial Krylov methods for the approximation of f(A)b, the action of a Stieltjes matrix function of a large Hermitian matrix on a vector. Using new error bounds and estimates, as well as existing results, we derive predictions of the practical performance of the methods, and rank them accordingly. As by-products, we derive new results on inexact Krylov iterations for matrix functions in order to allow for a fair comparison of rational Krylov methods with polynomial inner solves.

==> macros.tex <==

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\new}[1]{\textcolor{red}{#1}}
\newcommand{\newer}[1]{\textcolor{blue}{#1}}

%\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\blockdiag}{blockdiag}
\DeclareMathOperator{\Real}{Re} \DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\exterior}{ext}
\newcommand{\dist}{\text{dist}}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\hat}{\widehat}
\newcommand{\rangesp}[1]{{\mathcal R(#1)}}
\newcommand{\nullsp}[1]{\mathcal N(#1)}
\newcommand{\cond}[1]{\kappa(#1)}
\renewcommand{\angle}{{\measuredangle}}
\newcommand{\Grad}{{\nabla}}
%\newcommand{\diag}[1]{{\text{diag}(#1)}}
\renewcommand{\Re}{\text{Re}}
\renewcommand{\Im}{\text{Im}}
%\newcommand{\divdif}{\underset{/}{\Delta}}
%\newcommand{\divdif}{\Delta\kern-.68em/}
\newcommand{\divdif}{\mathord{\kern.43em{\vrule width.6pt height6pt depth-.28pt} \kern-.41em\Delta}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{assumption}{Assumption}
%{\theorembodyfont{\rmfamily}\newtheorem{rem}{Remark}}

%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{alg}{Algorithm}[section]
\newtheorem{example}{Example}[section]
%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]

%-------- Vectors

\newcommand{\va}{{\mathbf a}}
\newcommand{\vb}{{\mathbf b}}
\newcommand{\vc}{{\mathbf c}}
\newcommand{\vd}{{\mathbf d}}
\newcommand{\vdhat}{{\mathbf {\hat d}}}
\newcommand{\ve}{{\mathbf e}}
\newcommand{\vf}{{\mathbf f}}
\newcommand{\vg}{{\mathbf g}}
\newcommand{\vh}{{\mathbf h}}
\newcommand{\vhhat}{{\mathbf {\hat h}}}
\newcommand{\vk}{{\mathbf k}}
\newcommand{\vp}{{\mathbf p}}
\newcommand{\vq}{{\mathbf q}}
\newcommand{\vr}{{\mathbf r}}
\newcommand{\vs}{{\mathbf s}}
\newcommand{\vt}{{\mathbf t}}
\newcommand{\vu}{{\mathbf u}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\vw}{{\mathbf w}}
\newcommand{\vx}{{\mathbf x}}
\newcommand{\vy}{{\mathbf y}}
\newcommand{\vz}{{\mathbf z}}
\newcommand{\vnull}{\boldsymbol{0}}

\newcommand{\valpha}{\boldsymbol \alpha}

%---------- special iterates

\newcommand{\vcmr}{{\mathbf c}^{\text{MR}}}
\newcommand{\vcor}{{\mathbf c}^{\text{OR}}}
\newcommand{\vdor}{{\mathbf d}^{\text{OR}}}
\newcommand{\vdmr}{{\mathbf d}^{\text{MR}}}
\newcommand{\vdqmr}{{\mathbf d}^{\text{QMR}}}
\newcommand{\vdqor}{{\mathbf d}^{\text{QOR}}}
\newcommand{\vdme}{{\mathbf d}^{\text{ME}}}
\newcommand{\veor}{{\mathbf e}^{\text{OR}}}
\newcommand{\vemr}{{\mathbf e}^{\text{MR}}}
\newcommand{\veme}{{\mathbf e}^{\text{ME}}}
\newcommand{\vhor}{{\mathbf h}^{\text{OR}}}
\newcommand{\vhmr}{{\mathbf h}^{\text{MR}}}
\newcommand{\vhqmr}{{\mathbf h}^{\text{QMR}}}
\newcommand{\vhqor}{{\mathbf h}^{\text{QOR}}}
\newcommand{\vhme}{{\mathbf h}^{\text{ME}}}
\newcommand{\vror}{{\mathbf r}^{\text{OR}}}
\newcommand{\vrmr}{{\mathbf r}^{\text{MR}}}
\newcommand{\vrme}{{\mathbf r}^{\text{ME}}}
\newcommand{\vrqmr}{{\mathbf r}^{\text{QMR}}}
\newcommand{\vrqor}{{\mathbf r}^{\text{QOR}}}
\newcommand{\vrtfqmr}{{\mathbf r}^{\text{TFQMR}}}
\newcommand{\vrbcg}{{\mathbf r}^{\text{BCG}}}
\newcommand{\vrcgs}{{\mathbf r}^{\text{CGS}}}
\newcommand{\vsqmr}{{\mathbf s}^{\text{QMR}}}
\newcommand{\vvmr}{{\mathbf v}^{\text{MR}}}
\newcommand{\vvor}{{\mathbf v}^{\text{OR}}}
\newcommand{\vvqmr}{{\mathbf v}^{\text{QMR}}}
\newcommand{\vxor}{{\mathbf x}^{\text{OR}}}
\newcommand{\vxmr}{{\mathbf x}^{\text{MR}}}
\newcommand{\vxme}{{\mathbf x}^{\text{ME}}}
\newcommand{\vxqmr}{{\mathbf x}^{\text{QMR}}}
\newcommand{\vxqor}{{\mathbf x}^{\text{QOR}}}
\newcommand{\vxtfqmr}{{\mathbf x}^{\text{TFQMR}}}
\newcommand{\vxbcg}{{\mathbf x}^{\text{BCG}}}
\newcommand{\vxcgs}{{\mathbf x}^{\text{CGS}}}
\newcommand{\vyor}{{\mathbf y}^{\text{OR}}}
\newcommand{\vymr}{{\mathbf y}^{\text{MR}}}
\newcommand{\vyme}{{\mathbf y}^{\text{ME}}}
\newcommand{\vyqmr}{{\mathbf y}^{\text{QMR}}}
\newcommand{\vyqor}{{\mathbf y}^{\text{QOR}}}
\newcommand{\vwor}{{\mathbf w}^{\text{OR}}}
\newcommand{\vwmr}{{\mathbf w}^{\text{MR}}}
\newcommand{\vwhat}{\hat{\mathbf w}}
\newcommand{\vwqmr}{{\mathbf w}^{\text{QMR}}}
\newcommand{\vwqor}{{\mathbf w}^{\text{QOR}}}

\newcommand{\pmr}{p^{\text{MR}}}
\newcommand{\por}{p^{\text{OR}}}

% ---------- spaces

\newcommand{\cKm}{{\mathcal K}_m}
\newcommand{\spC}{{\mathcal C}}
\newcommand{\spH}{{\mathcal H}}
\newcommand{\spK}{{\mathcal K}}
\newcommand{\spP}{{\mathcal P}}
\newcommand{\spQ}{{\mathcal Q}}
\newcommand{\spT}{{\mathcal T}}
\newcommand{\spU}{{\mathcal U}}
\newcommand{\spV}{{\mathcal V}}
\newcommand{\spW}{{\mathcal W}}
\newcommand{\spZ}{{\mathcal Z}}

